Joint Inference of Diffusion and Structure in Partially Observed Social Networks Using Coupled Matrix Factorization

Access to complete data in large-scale networks is often infeasible. Therefore, the problem of missing data is a crucial and unavoidable issue in the analysis and modeling of real-world social networks. However, most of the research on different aspects of social networks does not consider this limitation. One effective way to solve this problem is to recover the missing data as a pre-processing step. In this paper, a model is learned from partially observed data to infer unobserved diffusion and structure networks. To jointly discover omitted diffusion activities and hidden network structures, we develop a probabilistic generative model called "DiffStru." The interrelations among links of nodes and cascade processes are utilized in the proposed method via learning coupled with low-dimensional latent factors. Besides inferring unseen data, latent factors such as community detection may also aid in network classification problems. We tested different missing data scenarios on simulated independent cascades over LFR networks and real datasets, including Twitter and Memtracker. Experiments on these synthetic and real-world datasets show that the proposed method successfully detects invisible social behaviors, predicts links, and identifies latent features.

==> images/properties.tex <==
\definecolor{normalnode}{rgb}{0.0, 1.0, 0.5}
\definecolor{uninfected}{rgb}{0.85, 0.75, 0.85} %{0.855, 0.957, 0.929}
\definecolor{infected}{rgb}{0.99, 0.54, 0.67}
\definecolor{fillcolor}{rgb} {0.98, 0.84, 0.65} %{0.82, 0.94, 0.75} %{0.63, 0.84, 0.71}

%\definecolor{c1}{HTML}{f69d9d}
%\definecolor{c2}{HTML}{b9e1dc}
\definecolor{c1}{rgb}{0.97, 0.51, 0.47}%{0.99, 0.42, 0.52} %{0.8, 0.9, 0.9}
\definecolor{c2}{rgb}{0.28, 0.82, 0.8}%{0.5, 1.0, 0.83} %{0.24, 0.82, 0.44} %{0.7, 0.8, 0.3}
\definecolor{c3}{rgb}{0.6, 0.0, 0.0} %{0.6, 0.7, 0.3}
%\definecolor{c4}{HTML}{537791}
\definecolor{c4}{rgb}{0.0, 0.27, 0.13}
\definecolor{plot}{rgb}{0.0, 0.33, 0.71}
\definecolor{bar1}{rgb}{0.98, 0.26, 0.62}
\definecolor{bar2}{rgb}{0.63, 0.36, 0.94}

\newcommand{\yslant}{0.5}
\newcommand{\xslant}{0}
\newcommand{\rad}{1cm}
\newcommand{\arrowColor}{c4}
\newcommand{\messageOneColor}{c1}
\newcommand{\messageTwoColor}{c2}


\tikzstyle{messageOne} = [pos=0.5, draw=\messageOneColor, fill=\messageOneColor, text width=7em, text=black, text centered, rounded corners, font=\tiny]

\tikzstyle{messageTwo} = [pos=0.5, draw=\messageTwoColor, fill=\messageTwoColor, text width=7em, text=black, text centered, rounded corners, font=\tiny]



==> images/truth-observed.tex <==
\usetikzlibrary{calc}

\tikzset{
	latent/.style={draw, minimum width=8mm, shape=circle, ultra thick, black}
}
\tikzset{
	auxiliary/.style={draw,dashed, minimum width=8mm, shape=circle, ultra thick, black}
}

\input{./images/properties.tex}
\begin{tikzpicture}[scale = 1, font=\small]
\node at (8.2, 4) {\textbf{Ground Truth}};
\node at (8.2, -2) {\textbf{Observed}};
\node at (-1.5, -7) {\textbf{Structure}};
\node at (5, -7) {\textbf{Cascade}};

\begin{scope}[
xshift=-120,
every node/.append style={yslant=\yslant,xslant=\xslant, font=\bf},yslant=\yslant,xslant=\xslant]
 
\draw[black, dashed, thin, fill=fillcolor] (0,0) rectangle (5,5); 

\draw [->, ultra thick] (1.5, 0.7) to [out=3-30, in=180+30] (3.5, 0.7);
\draw [->, ultra thick] (1.98, 2.3) to [out=180, in=90](1.3, 1.5);
\draw [->, ultra thick] (3, 2.2) to [out=-30, in=90+15](3.6, 1.4);
\draw [->, ultra thick] (2.9, 2.9) to [out=0, in=-90](3.6, 3.6);
\draw [->, ultra thick] (1.3, 4.5) to [out=30, in=180-30] (3.6, 4.5);
\draw [->, ultra thick] (1.3, 3.5) to [out=-60, in=180-30](2.05, 2.9);

\draw [fill = normalnode, ultra thick] (1, 1) circle (0.5) node {A};
\draw [fill = normalnode, ultra thick] (4, 1) circle (0.5) node {B};
\draw [fill = normalnode, ultra thick] (2.5, 2.5) circle (0.5) node [thick] {C};
\draw [fill = normalnode, ultra thick] (4, 4) circle (0.5) node {D};
\draw [fill = normalnode, ultra thick] (1, 4) circle (0.5) node {E};

\draw[thin] (1, 4) -- (7.5, 0.7);
\draw[thin] (1, 1) -- (7.5, -2.3);
\draw[thin] (2.5, 2.5) -- (9, -0.8);
\draw[thin] (4, 4) -- (10.5, 0.7);
\draw[thin] (4, 1) -- (10.5, -2.3);
\end{scope}

\begin{scope}[
yshift=0,
xshift=60,
every node/.append style={yslant=\yslant,xslant=\xslant},
yslant=\yslant,xslant=\xslant
] 
\draw[black, dashed, thin] (0,0) rectangle (5,5); 
\fill[fillcolor,fill opacity=.75] (0,0) rectangle (5,5);

\draw [fill = infected, ultra thick, font=\bf] (1, 1) circle (0.5) node {A};
\node at (1, 1.75) {t=0.23};
\draw [fill = infected, ultra thick, font=\bf] (4, 1) circle (0.5) node {B};
\node at (4, 1.75) {t=0.00};
\draw [fill = infected, ultra thick, font=\bf] (2.5, 2.5) circle (0.5) node {C};
\node at (2.5, 3.25) {t=0.28};
\draw [fill = uninfected, ultra thick, font=\bf] (4, 4) circle (0.5) node {D};
\draw [fill = infected, ultra thick, font=\bf] (1, 4) circle (0.5) node {E};
\node at (1, 4.75) {t=0.42};
\end{scope}

\begin{scope}[
yshift=-180,
xshift=-120,
every node/.append style={yslant=\yslant,xslant=\xslant, font=\bf},
yslant=\yslant,xslant=\xslant
] 
\draw[black, dashed, thin] (0,0) rectangle (5,5); 
\fill[fillcolor,fill opacity=.75] (0,0) rectangle (5,5);

%	\draw [thin] (1, 1) to (4, 1);
%	\draw [thin] (2.5, 2.5) to (4, 1);
%	\draw [thin] (2.5, 2.5) to (4, 4);

\draw [fill = normalnode, ultra thick] (1, 1) circle (0.5) node {A};
\draw [fill = normalnode, ultra thick] (4, 1) circle (0.5) node {B};
\draw [fill = normalnode, ultra thick] (2.5, 2.5) circle (0.5) node {C};
\draw [fill = normalnode, ultra thick] (4, 4) circle (0.5) node {D};
\draw [fill = normalnode, ultra thick] (1, 4) circle (0.5) node {E};

\draw [->, ultra thick] (1.5, 0.7) to [out=3-30, in=180+30] (3.5, 0.7);
\draw [->, ultra thick] (1.98, 2.3) to [out=180, in=90](1.3, 1.5);
%	\draw [->, thin] (3, 2.2) to [out=-30, in=90+15](3.6, 1.4);
\draw [->, ultra thick] (2.9, 2.9) to [out=0, in=-90](3.6, 3.6);
%	\draw [->, thin] (1.3, 4.5) to [out=30, in=180-30] (3.6, 4.5);
%	\draw [->, thin] (1.3, 3.5) to [out=-60, in=180-30](2.05, 2.9);

\end{scope}

\begin{scope}[
yshift=-180,
xshift=60,
every node/.append style={yslant=\yslant,xslant=\xslant},
yslant=\yslant,xslant=\xslant
] 
\draw[black, dashed, thin, fill=fillcolor] (0,0) rectangle (5,5); 

\draw [fill = infected, ultra thick, font=\bf] (1, 1) circle (0.5) node {A};
\node at (1, 1.75) {t=0.23};
\draw [fill = infected, ultra thick, font=\bf] (4, 1) circle (0.5) node {B};
\node at (4, 1.75) {t=0.00};
\draw [fill = uninfected, ultra thick, font=\bf] (2.5, 2.5) circle (0.5) node {C};
\draw [fill = uninfected, ultra thick, font=\bf] (4, 4) circle (0.5) node {D};
\draw [fill = infected, ultra thick, font=\bf] (1, 4) circle (0.5) node {E};
\node at (1, 4.75) {t=0.42};
\end{scope}


\end{tikzpicture}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Auxiliary node
\tikzstyle{auxiliary} = [circle,fill=white,draw=black,dashed,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

